FLIPHAT: Joint Differential Privacy for High Dimensional Sparse Linear Bandits

High dimensional sparse linear bandits serve as an efficient model for sequential decision-making problems (e.g. personalized medicine), where high dimensional features (e.g. genomic data) on the users are available, but only a small subset of them are relevant. Motivated by data privacy concerns in these applications, we study the joint differentially private high dimensional sparse linear bandits, where both rewards and contexts are considered as private data. First, to quantify the cost of privacy, we derive a lower bound on the regret achievable in this setting. To further address the problem, we design a computationally efficient bandit algorithm, \textbf{F}orgetfu\textbf{L} \textbf{I}terative \textbf{P}rivate \textbf{HA}rd \textbf{T}hresholding (FLIPHAT). Along with doubling of episodes and episodic forgetting, FLIPHAT deploys a variant of Noisy Iterative Hard Thresholding (N-IHT) algorithm as a sparse linear regression oracle to ensure both privacy and regret-optimality. We show that FLIPHAT achieves optimal regret in terms of privacy parameters $\epsilon, \delta$, context dimension $d$, and time horizon $T$ up to a linear factor in model sparsity and logarithmic factor in $d$. We analyze the regret by providing a novel refined analysis of the estimation error of N-IHT, which is of parallel interest.

==> body.tex <==
\section{INTRODUCTION}
Multi-armed bandits, in brief \textit{bandits}, constitute an archetypal model of sequential decision-making under partial information~\citep{lattimore2018bandit}. In bandits, a learner sequentially chooses one decision from a collection of actions (or arms). In return, it observes only the reward corresponding to the chosen action with the goal of maximizing the accumulated rewards over a time horizon.
Additionally, the available decisions at any point of interaction might depend on some side information about the actions, encoded as a feature vector. In linear contextual bandits (LCB) \citep{auer2002using,abe2003reinforcement}, the learner observes such a feature vector (aka \textit{context}) for each action before taking a decision, and the rewards are generated by a linear function of the chosen context and an unknown parameter vector. 
LCBs are widely studied and deployed in real-life applications, such as online advertising~\citep{schwartz2017customer}, recommendation systems~\citep{silva2022multi}, investment portfolio design~\citep{silva2022multi}, and personalized medicine~\citep{peng2021machine}. 

In many of these applications, the personal information used as contexts often has a large dimension, which can be modeled by viewing the contexts as high-dimensional vectors. This is relevant in the modern big data era, where the applications usually deal with many features. However, the established regret lower bound in LCB polynomially depends on the context dimension~\citep{dani2008stochastic, chu2011contextual}. Thus, additional structural conditions, such as sparsity, are needed to be enforced to make the problem tractable. Sparsity aligns with the idea that among these features, possibly only a small subset of them are relevant to generate the reward. This setting is called the \textit{high-dimensional sparse linear contextual bandit} (SLCB). Recently, SLCB has received significant attention~\citep{wang2018minimax,bastani2020online,HaoLattimore2020,chakraborty2023thompson} and have been useful in practical applications~\citep{miao2022online,ren2024dynamic}.

\textbf{Data Privacy in SLCB.} We observe that the applications of SLCB, e.g. recommender systems and personalized medicines, involve sensitive data of individuals. This naturally invokes data privacy concerns and requires development and analysis of data privacy-preserving SLCB algorithms. 

\textit{Example 1.} One of the earliest successful application of linear contextual bandits is personalized news article recommendation and its validation on Yahoo! Today Module by~\citet{li2010contextual}. In the dataset collected from Yahoo! platform, each user is represented by a 1193-dimensional features but for a successful deployment they are reduced to 5 dimensions. 
The feature of every user include their gender, age, geographical address, and even behavorial quantifiers. 
These are sensitive data as per GDPR~\citep{voigt2017eu} and California Consumer Privacy Act~\citep{ccpa}. Thus, protecting data privacy in this problem, and designing efficient and private SLCB algorithms are fundamentally necessary.

\textit{Example 2.} A recent example of deploying SLCB with user-data is optimizing click-through rates in the Tencent search advertising
dataset~\citep{tencent}. Though each context is 509256 dimensional, it lends itself to a sparse structure~\citep{wangtencent}. 
Here, also the context incorporates sensitive information, like gender, age etc., which are protected by privacy laws. Thus, private SLCBs are a natural requirement here.

\textit{Example 3.} %\begin{example}%\label{ex:1}
Another application of SLCB is a mobile health application that recommends a personalized treatment plan (actions) to each patient (user) based on her personal information, such as age, weight, height, medical history etc.~\citep{tewari2017ads,killian2023robust}. %The recommendations to the users are obtained as feedback through an interactive portal. 
% Here, for every user $u$ and personalized treatment plan $a$ contexts are obtained via a feature representation $x=\phi(u, a)\in\bbR^d$~\citep{shariff2018differentially}. For example, 
Here, for every user and personalized treatment plan contexts are generally obtained through a feature representation, where the dimension is often large but there are only fewer relevant features. %Here, $d$ is often large to capture the complex interactions across treatment plans and user information but there are fewer $s^{*}$ features that finally impact the treatment outcomes.
%Once the recommendation algorithm provides a treatment plan, it induces a change in the users medical condition.
% The goal of the recommendation algorithm is to improve the medical condition of the users as much as possible over a number of interactions.
% Meanwhile, this mobile app’s recommendation algorithm %also needs to be updated once in a while in a cloud server after collecting feedback data from a batch of patients. 
The algorithm uses patients' data including treatment outcomes and medical contexts of patients, which are sensitive information as per GDPR, CCPA, and HIPAA~\citep{annas2003hipaa}. Hence, this is a natural application that motivates the study of efficient and privacy-preserving SLCB algorithms.
% each patient would like to obtain a personalized and effective treatment plan while demanding their private information remain protected against an adversary.
% \end{example}

\textbf{Related Work: Differential Privacy in Bandits.} Problems like the ones in the aforementioned examples motivate us to study data-privacy preserving SLCB algorithms. Specifically, we follow Differential Privacy (DP)~\citep{dwork2006differential} as the data privacy framework. DP aims to ensure that while looking into the output of an algorithm, an adversary is unable to conclude whether a specific user was in the input dataset. DP has emerged as the gold standard of data privacy. It has been extensively studied in various domains with the goal of safe-guarding sensitive data from adversarial attacks~\citep{dwork2014algorithmic,Abadi_MomentAccountant,McMahan_Privacy}.
Impact of DP and designing efficient DP-preserving algorithms have also been studied for different settings of bandits, such as stochastic bandits~\citep{Mishra2015NearlyOD, tossou2016algorithms, sajed2019optimal, hu2022near,azize2022privacy_dpband}, adversarial bandits~\citep{tossou2017achieving} and LCB~\citep{shariff2018differentially,neel2018mitigating, hanna2024differentially,azize2023privacy}. 

The literature also reveals that different notions of DP are possible in bandits depending on what we consider as the sensitive input to be saved and what are the public output. In comparison to the supervised learning literature, additional difficulties arise due to the complex interaction between the policy employed by the learner, and the stochastic nature of the contexts and rewards. \textit{Local}~\citep{duchi2013localextended} and \textit{global} \citep{basu2019differential} definitions of DP are extended to bandits, where we aim to keep the rewards generated during interactions private.
In local DP, users already send to the learner privatized rewards as feedback. In global DP, the learner gets true rewards but it publishes actions in a way that the rewards stay private.
For LCBs, compared to reward privacy, \cite{shariff2018differentially} study a stronger form of privacy that aims to keep both the rewards and the contexts private while publishing the actions. This is called Joint Differential Privacy (JDP), which is further strengthened by~\cite{vietri2020private}. 
In this paper, \textit{we follow $(\epsilon, \delta)$-JDP of \citep{vietri2020private} as our privacy framework}, since it best aligns with our interest of protecting both users' information and the outcomes collected over all the interactions.

We observe that though there are multiple algorithms for  $(\epsilon, \delta)$-JDP (Definition~\ref{def: JDP}) satisfying LCBs, they are tailored for the low dimensional setting and scales polynomially with the context dimension $d$. In contrast, the study of JDP in SLCB setting is still unexplored. This leads us to two questions:\\
% \begin{enumerate}[leftmargin=*]
1. \textit{What is the cost of ensuring $(\epsilon, \delta)$-JDP in high-dimensional sparse linear contextual bandits?}\\
2. \textit{Can we design a privacy-preserving SLCB algorithm that achieves the minimal cost due to $(\epsilon, \delta)$-JDP?}
% \end{enumerate}

\textbf{Contributions.} Our study of these questions leads us to the following contributions.

% \begin{enumerate}[leftmargin=*]
    1. \textit{Regret Lower Bound}:
    % The lower bound on regret achievable by any algorithm quantifies the hardness of a bandit problem. 
    We derive a {  \textit{problem independent}} regret lower bound for SLCBs with $(\epsilon,\delta)$-JDP. Our lower bound demonstrates a phase transition between the hardness of the problem depending on the privacy level, similar to~\citep{azize2023privacy} (reward-private low-dimension LCB).
    Compared to linear dependence on $d$ \citep{azize2023privacy}, our lower bound depends linearly on { {$\sqrt{s^*} \log d$}} for a fixed privacy budget, where $s^*$ is the problem sparsity parameter and $d$ is the context dimension.
    %But our lower bound shows a linear dependence on $s^{*}\log d$ than $d$, which is ideally the effective dimension in SLCB setting. Here, $s^{*}$ is called the sparsity level.
    %While regret lower bound for linear contextual bandits have been studied \citep{li2021regret}, the proof technique cannot be modified to our setting because of the privacy restriction on the space of policies.
    
    2. \textit{Algorithm and Regret Analysis}: We propose a novel SLCB algorithm, namely FLIPHAT, that uses N-IHT as a key component, and prove its $(\epsilon,\delta)$-JDP guarantee. We analyze the expected regret for FLIPHAT and demonstrate that in the problem-independent case, the upper bound matches our lower bound up to  { {$s^*$} and} logarithmic factors in $T$. We also numerically demonstrate its logarithmic dependence on $d$ across privacy regimes.
   
    3. \textit{Interaction of Privacy and Hardness of Bandit:} In Theorem \ref{thm: regret}, we identify a unique interplay between two competing hardness: privacy and the internal hardness of the bandit instance. We show that as the internal hardness of bandit decreases, the hardness due to privacy becomes more prevalent and persists for wider (and larger) values of the privacy parameters, and vice-versa. To the best of our knowledge, this is a previously unidentified phenomenon, and demands careful understanding.

     4. \textit{Improved analysis of N-IHT}: We provide a refined analysis for Peeling-based~\citep{dwork2021differentially} empirical risk minimization under non i.i.d. setting. This yields a bound on estimation error of N-IHT under the SLCB setting, and it is used in the regret analysis of FLIPHAT. The results and tools developed here might be of independent interest and can be applied in settings where N-IHT is deployed.

% \end{enumerate}


% \paragraph{Notations} 

% Let $\bbR$ and $\bbR^+$ denote the set of real numbers and the set of non-negative real numbers respectively. Denote by $\bbR^d$ the $d$-dimensional Euclidean space. For a positive integer $K$, denote by $[K]$ the set $\{1, 2, \ldots, K\}$. 
% Regarding vectors and matrices, for a vector $v \in \bbR^d$, we denote by $\norm{v}_0, \norm{v}_1,\norm{v}_2, \norm{v}_\infty$ the $\ell_0, \ell_1, \ell_2, \ell_\infty$ norms of $v$ respectively. For a $p\times q$ matrix $M$  we define the $\norm{M}:= \max_{j \in [q]} \sqrt{(M^\top M)_{j,j}}$. 
% Regarding random variables, $\norm{Z}_{\psi_2}$ denotes the Orlicz norm of the random variable $Z$, i.e., $\norm{Z}_{\psi_2} = \inf \{\lambda >0 : \bbE \exp(Z^2/\lambda^2) \leq 2\}$. For a random vector $X\in \bbR^p$, the corresponding Orlicz norm is defined as $\norm{X}_{\psi_2}:= \sup_{u \in \bbS^{p-1}} \norm{u^\top X}_{\psi_2}$. We denote $\cO, \Omega$ as the usual big-oh and Omega functions to capture asymptotic behavior and $\tilde{\cO}$ 
% Throughout the paper, let $O(\cdot)$ denote the standard big-O notation, i.e., we say $a_n = O(b_n)$ if there exists a universal constant $C>0$, such that $a_n \leq C b_n$ for all $n \in \mathbb{N}$. Sometimes for notational convenience, we write $a_n \lesssim b_n$ in place of $a_n = O(b_n)$. We write $a_n \asymp b_n$ or $a_n = \Theta(b_n)$ if $a_n = O(b_n)$ and $b_n = O(a_n)$.
\section{PROBLEM FORMULATION}\label{sec: problem}%: Sparse Linear Contextual Bandit with JDP}\label{sec: problem}
%\textbf{Notations.} $[K]$ denotes the set $\{1,\ldots, K\}$.
%$\Delta_K$ is the simplex on $[K]$.

A high-dimensional \textit{sparse linear stochastic contextual bandit (SLCB)} consists of $K\in \mathbb{N}$ arms. At time $t\in [T]$\footnote{For $K \in \bbN$, $[K]$ denotes the set $\{1, \ldots, K\}$.}, context vectors $\{x_i(t)\}_{i\in [K]}$ are revealed for every arm $i$. 
For every $i\in[K]$, we assume $x_i(t)\in \bbR^d$, and are sampled i.i.d.\ from some unknown distribution $P_i$. 
% Moreover, we specifically consider the high-dimensional setting $T\ll d$, i.e., the time horizon T (possibly unknown) is much smaller compared to the ambient dimension.
At every step $t$, an action $a_t \in [K]$ is chosen by the learner and a noisy reward $r(t)$ is obtained through a linear model:
\begin{align}\label{eq: base model}
    r(t) = x_{a_t}(t)^\top \beta^* + \epsilon(t)\,.
\end{align}
Here, $\beta^*\in\bbR^d$ is the unknown true signal, which is $s^*$-sparse i.e., $\norm{\beta^*}_0 = s^*$ with $s^* \ll d$. $\{\epsilon(t)\}_{t\in[T]}$ are independent sub-Gaussian noise, which are independent of all the other processes. Furthermore, we assume boundedness assumption on the contexts and parameter, i.e., $\norm{x_i(t)}_\infty \le \xmax \;\forall (i,t) \in [K]\times [T]$ almost surely, and $\norm{\beta^*}_1 \le \bmax$. Such assumptions are common in prior LCB literature, \citep{HaoLattimore2020, li2021regret, azize2023privacy} and are crucial for privacy guarantees.

Now, to formalize the notion of performance of a learner, we define the best action in hindsight at the step $t$ as $a_t^*:= \argmax_{i \in [K]} x_i(t)^\top \beta^*$. Then, the goal is to design a sequential algorithm (policy) $\pi$. At each step $t$, $\pi$ takes the observed reward-context pairs until time $t-1$ as input and outputs a distribution $\pi_t$ over the action space $[K]$. The learner selects an action $a_t\sim \pi_t$ using the policy $\pi$. Then, we define regret of policy $\pi$ as\footnote{We sometimes drop the subscript $\pi$ in regret, when the dependence of on the policy is clear from context.} 
\begin{align}\label{eq:regret}
    R_{\pi}(T) := \sum\nolimits_{t \in [T]} \left[x_{a_t^*}(t)^\top \beta^* - x_{a_t}(t)^\top \beta^*\right]\, .
\end{align}
The goal of the learner is to construct a SLCB policy $\pi$ to maximize the cumulative reward till time $T$, or equivalently, minimize $R_{\pi}(T)$.

\textbf{Joint DP for SLCB.} Now, we concretely define the notion of DP in SLCB. 
It is well known that the original notion of DP~\citep{dwork2006calibrating} is not ideal in contextual bandit setting due to the inevitability of linear regret~\citep[Claim 13]{shariff2018differentially}.
Therefore, we consider the notion of JDP~\citep{vietri2020private}. In JDP, both rewards and contexts are considered as sensitive information about the users which are used by $\pi$ as input and should be kept private from any external adversary. 

To formalize further, let us denote by $\br_t:= (r_1(t), \ldots, r_K(t))$ the collection of rewards, and $\cC_t:= (x_1(t), \ldots, x_K(t))$ the collection of user contexts at time $t$. At the beginning of the game, the adversary prefixes the whole collection of rewards $\{\br_t\}_{t \in [T]}$ and contexts $\{\cC_t\}_{t\in [T]}$.  
%Similarly, $\cC_t:= (x_1(t), \ldots, x_K(t))$ be the user contexts corresponding to the arms. 
In the $t$-th step, the learner observes the contexts $\cC_t$ and chooses an action $a_t$ using only the past \textit{observed} rewards and contexts. Then, adversary reveals the reward $r_{a_t}(t)$ and the game continues.
Under this paradigm, one can define the whole input dataset as the collection of all the rewards and contexts. Specifically, we consider $\cD:= \{(\br_t, \cC_t)\}_{t \in [T]}$ as the input data to a bandit algorithm $\cA$.  
A randomized bandit algorithm $\cA$ maps every reward-context sequence $\cD$ of length $T$ to a (random) sequence of actions $a:=(a_1,\dots,a_T)\in [K]^T$. Therefore, $\cA(\cD)$ can be imagined as a random vector taking values in $[K]^T$. %(as $[K]$ is our action space for each time point)
Let $\cA_{-t}(\cD)$ denote all the outputs excluding the output in the $t$-th step of the interaction of $\cA$ with the bandit instance. 
$\cA_{-t}(\cD)$ captures all the outputs that might leak information about the user at the $t$th time point in interactions after the $t$th round, as well as all the outputs from the previous episodes where other users could be submitting information to the agent adversarially to condition its interaction with the $t$th user. Finally, we say that two input datasets $\cD$ and $\cD^\prime := \{(\br^\prime_t, \cC^\prime_t)\}_{t \in [T]}$ are $\tau$-neighbors, if for all $t \ne \tau$ we have $(\br_t, \cC_t) = (\br^\prime_t, \cC^\prime_t)$, and $(\br_\tau, \cC_\tau) \ne (\br^\prime_\tau, \cC^\prime_\tau)$.
\begin{definition}[JDP in LCB]
\label{def: JDP}
    A randomized bandit algorithm $\cA$ is $(\epsilon, \delta)$-JDP if for any $\tau \in [T]$ and any pair of $\tau$-neighboring sequences $\cD$ and $\cD^\prime$, and any subset $E\subset [K]^{T-1}$, it holds that  $$\pr(\cA_{- \tau}(\cD) \in E) \le e^\epsilon \pr(\cA_{- \tau}(\cD^\prime) \in E) + \delta.$$
    % where for $\cA(S)=(a_1,\dots,a_T)$, we denote $\cA(S)_{\neq \tau} = (a_1,\dots,a_{\tau-1},a_{\tau+1},\dots,a_T)$, i.e., leaving the $\tau-$th time point.
\end{definition}
Although the above JDP definition is valid for any randomized contextual bandit algorithm $\cA$,
it is useful to point out that in our setup, the bandit protocol $\cA$ is solely defined by the inherent policy $\pi$. 
% \paragraph{Problem Statement:} The goal of this paper is to explore the area of high-dimensional SLCB under JDP setting. In particular, we prove a minimax regret lower bound result and propose a novel algorithm that enjoys a nearly-matching regret upper bound. 

% \begin{table}[t]
%   \caption{Comparison with prior works on private LCB (under no-margin condition)}
%   \label{table: prior work}
%   \small
%   \centering
%   \begin{tabular}{lllll}
%     \toprule
%     % \multicolumn{2}{c}{Part}                   \\
%     % \cmidrule(r){1-2}
%          & Settings & parameter & Context & Regret Bound\\
%     \midrule
%     % \cite{dani2008stochastic} & LCB, $\beta^*$ & fixed  & $\tilde{\cO}(d\sqrt{T})$\\
%     % \cite{agrawal2013thompson} & LCB, $\beta^*$ & stochastic  & $\tilde{\cO}\left(d^2\sqrt{T^{1+\epsilon}}/\epsilon\right)$\\
%     % \cite{chu2011contextual} & LCB, $\beta^*$ & stochastic  & $\tilde{\cO}(\sqrt{dT})$\\
%     % \cite{bastani2020online} & Sparse LCB, $\beta_i^*$  & stochastic  & $\cO\left(s^2[\log T + \log d]^2\right)$     \\
%     % \cite{HaoLattimore2020} & Sparse LCB, $\beta^*$ & stochastic & $\cO(T^{2/3}\log d)$\\
%     % \cite{li2021regret} & Sparse $\beta^*$ & stochastic  & $\cO\left(\sqrt{T\log d} + \log T\right)$\\
%     % \cite{chakraborty2023thompson} & Sparse LCB, $\beta^*$ & stochastic & $\cO(s^2[\log d + \log T]$\\


%     \cite{shariff2018differentially}(lb) & LCB + JDP  & single & adversarial & $\tilde{O}(d \sqrt{T/\epsilon})$\\
%     \cite{zheng2020locally} & LCB + LDP & single & adversarial & $\tilde{O}((dT)^{3/4}/\epsilon)$\\
%     \cite{han2021generalized}(lb) & LCB + LDP & single/ multiple & stochastic & $\tilde{O}(d^{3/2}\sqrt{T/\epsilon})$\\
%     \cite{garcelon2022privacy} & LCB + JDP & single & adversarial & $\tilde{O}(dT^{2/3}/\epsilon^{1/3})$\\
%     \cite{hanna2024differentially} & LCB + reward-DP & single & adversarial & $\tilde{O}(d \sqrt{T} + d^2/\epsilon)$ \\
%     \cite{chowdhury2022shuffle} & LCB + LDP& single & adversarial & $\tilde{O}(d T^{3/5} + d^{3/4}T^{3/5}/\epsilon^{1/2})$\\\cite{azize2023privacy}(lb) & LCB + reward-DP & single & stochastic & $\tilde{O}(\sqrt{dT} + d/\epsilon)$ \\
%     \textbf{This paper} & \textbf{Sparse LCB + JDP} & single  & stochastic & $\tilde{O}(s^*\sqrt{T \log d} \vee (s^{* 3/2} \log d)/\epsilon)$\\
%     \bottomrule
%   \end{tabular}
% \end{table}

\begin{table*}[t]
  \caption{Comparison with prior works on private LCB (under no-margin condition)}
  \label{table: prior work}
  %\small
  \centering
  \small{
  \begin{tabular}{llll}
    \toprule
    % \multicolumn{2}{c}{Part}                   \\
    % \cmidrule(r){1-2}
        Paper & Settings & Contexts  & Regret Bound\\
    \midrule
    % \cite{dani2008stochastic} & LCB, $\beta^*$ & fixed  & $\tilde{\cO}(d\sqrt{T})$\\
    % \cite{agrawal2013thompson} & LCB, $\beta^*$ & stochastic  & $\tilde{\cO}\left(d^2\sqrt{T^{1+\epsilon}}/\epsilon\right)$\\
    % \cite{chu2011contextual} & LCB, $\beta^*$ & stochastic  & $\tilde{\cO}(\sqrt{dT})$\\
    % \cite{bastani2020online} & Sparse LCB, $\beta_i^*$  & stochastic  & $\cO\left(s^2[\log T + \log d]^2\right)$     \\
    % \cite{HaoLattimore2020} & Sparse LCB, $\beta^*$ & stochastic & $\cO(T^{2/3}\log d)$\\
    % \cite{li2021regret} & Sparse $\beta^*$ & stochastic  & $\cO\left(\sqrt{T\log d} + \log T\right)$\\
    % \cite{chakraborty2023thompson} & Sparse LCB, $\beta^*$ & stochastic & $\cO(s^2[\log d + \log T]$\\


    \cite{shariff2018differentially} & LCB + JDP  & adversarial & $\tilde{O}(d \sqrt{T/\epsilon})$\\
    \cite{zheng2020locally} & LCB + LDP & adversarial & $\tilde{O}((dT)^{3/4}/\epsilon)$\\
    \cite{han2021generalized} & LCB + LDP  & stochastic & $\tilde{O}(d^{3/2}\sqrt{T/\epsilon})$\\
    \cite{garcelon2022privacy} & LCB + JDP & adversarial & $\tilde{O}(dT^{2/3}/\epsilon^{1/3})$\\
    \cite{hanna2024differentially} & LCB + reward-DP & adversarial & $\tilde{O}(d \sqrt{T} + d^2/\epsilon)$ \\
    \cite{chowdhury2022shuffle} & LCB + LDP & adversarial & $\tilde{O}(d T^{3/5} + d^{3/4}T^{3/5}/\epsilon^{1/2})$\\\cite{azize2023privacy} & LCB + reward-DP & stochastic & $\tilde{O}(\sqrt{dT} + d/\epsilon)$ \\
    \textbf{This paper} & \textbf{Sparse LCB + JDP}   & stochastic & $\tilde{O}(s^*\sqrt{T \log d} \vee (s^{* 3/2} \log d)/\epsilon)$\\
    \bottomrule
  \end{tabular}}
\end{table*}

% Table \ref{table: prior work} gives a brief idea on the vast literature on LCB, SLCB and LCB under JDP - note that the upper bounds should be compared with care since they are derived under slightly different settings and assumptions. It is worthwhile to point out that two different settings have been popular for LCB - works like \cite{bastani2020online, wang2018minimax} consider different $\beta_i^*$ for each arm $i\in[K]$ with a single context $x_t$ per round, our formulation aligns with those in \cite{li2021regret, agrawal2013thompson}, where $K$ contexts are revealed and there is only one $\beta^*$. Some works like \cite{abbasi2011improved, dani2008stochastic} consider infinitely many actions and the latter and other authors \cite{hao2021information} consider the case where the set of contexts is fixed over $t$, thereby leading to a fixed optimal arm across all rounds. Other notable work in SLCB include \cite{kim2019doubly}, \cite{oh2021sparsity, chakraborty2023thompson}, and \cite{shariff2018differentially, basu2019differential_dpband} for JDP in LCB. We remark that to our knowledge, the current paper is the first work to study JDP in the sparse linear contextual bandit setting. { {check references. add lower bound references}}
\textbf{Connection with Prior Works on Private LCB.} 
%Privacy in the LCB setting has been studied in several prior works under different notions of DP. 
\cite{shariff2018differentially} first studied LCB under $(\epsilon,\delta)$-JDP. Their proposed UCB-based algorithm enjoys $\tilde{O}(d\sqrt{T/\eps
})$\footnote{$\tilde{O}(\cdot)$ hides the poly-logarithmic dependence in $T$ and $d$.} regret bound. However, \textit{their notion of JDP is slightly weaker as it only considers the privacy of future actions}. \cite{garcelon2022privacy} considered a stronger definition of JDP (same as Definition \ref{def: JDP}), and proposed an algorithm with $\tilde{O}(d T^{2/3}/\epsilon^{1/3})$ regret. Still, achieving the known lower bound under JDP~\citep{he2022reduction}, i.e. $\Omega(\sqrt{dT\log K} + \frac{d}{\epsilon+\delta})$, is an open question. 
%This is a better regret guarantee than that of \cite{shariff2018differentially}, when $\epsilon = O(T^{-1/2})$. 
There is a parallel line of works~\citep{zheng2020locally, han2021generalized, chowdhury2022distributed} that considers Local Differential Privacy (LDP) under the LCB setting. LDP is a much stronger notion of privacy compared to the central nature of JDP. Therefore, the algorithms under LDP typically suffer a worse regret guarantee, i.e. $\Omega(\sqrt{dT}/\eps)$. %However, the algorithm of \cite{han2021generalized} matches the lower bound $\Omega(\sqrt{dT}/\eps)$ (in terms of $T$). 
In another stream, \cite{hanna2024differentially} and \cite{azize2023privacy} considered the reward-DP model under the LCB setting, which only aims to privatize the reward stream. Under an adversarial (contexts) setting, \cite{hanna2024differentially}  obtains $\tilde{O}(d \sqrt{T} + d^{2}/\epsilon)$, and \cite{azize2023privacy} obtains $\tilde{O}(\sqrt{dT} + d/\epsilon)$ regret under stochastic setting that matches the lower bound. However, all these algorithms suffer a polynomial dependence in $d$, i.e. $\Omega(\sqrt{d})$ in non-private term and $\Omega(d)$ in private term, which are not desirable in high-dimension. In our work, we propose a novel algorithm under the SLCB setting that only scales poly-logarithmically on the dimension $d$ under JDP (ref. Table \ref{table: prior work}). Moreover, our regret upper and lower bounds demonstrate a phase transition in the regret in the SLCB setting under JDP, similar to \citep{garcelon2022privacy,azize2022privacy}.


%\subsection{Assumptions}
% We briefly discuss the assumptions that we impose on the various model components - such assumptions are well accepted in the literature on SLCB \citep{zhang2008sparsity, zhang2010nearly, bastani2020online, li2021regret, chakraborty2023thompson}. \textit{We note that no additional assumption is enforced to capture the privacy requirements, apart from only those required for SLCB.} 

% \begin{definition}[Sparse Riesz Condition]
% \label{def: sparse eigen value}
% For a $d\times d$ positive semi-definite matrix $A$, its maximum and minimum sparse eigenvalues with parameter $s\in [d]$ are defined as $\phi_{\min}(s; A):= \inf_{u: u \neq 0, \norm{u}_0 \leq s} u^\top A u /\norm{u}_2^2, \quad \phi_{\max}(s; A) := \sup_{u: u \neq 0, \norm{u}_0 \leq s} u^\top A u/\norm{u}_2^2$.
% % We say $A$ has Sparse Riesz Condition if  $0< \phi_{\min}(s, A) \leq \phi_{\max}(s; A) < \infty$.
% \end{definition}

% \begin{assumption}[Assumptions on Context Distributions] \label{assumptions: contexts}
% We assume that
% \begin{enumerate}[label=(\alph*),leftmargin=*]
% \itemsep0em
%     \item \label{item: context_bound} \textit{Boundedness:} $\bbP_{x\sim \cP_i} (\norm{x}_\infty \leq \xmax) =1$ for all $i\in[K]$ for a constant $\xmax\in \bbR^+$.
%     \item \label{item: context_subgaussian} \textit{Bounded Orlicz norm:} For all arms $i \in [K]$ the distribution $\cP_i$ is bounded in the Orlicz norm, i.e., $\norm{X}_{\psi_2}\leq \vartheta$ for $X\sim \cP_i$ for all $i\in [K]$. %\sapta{may use new line for equation}
%     \item \label{item: anti-concentration} \textit{Anti-concentration:} There exists a  constant $\xi\in \bbR^+$ such that for each $u\in \{v\in\bbR^d : \norm{v}_0 \leq Cs^*, \norm{v}_2=1\}$ and $h\in \bbR^+$ 
%     $\cP_i(\innerprod{x, u}^2 \leq h) \leq \xi h,$
%     for all $i\in [K]$, ,where $C\in (2,\infty)$.
%     \item \label{item: sparse_eigenvalue} \textit{Sparsity:} The matrix $\Sigma_i := \bbE_{x\sim \cP_i} [x x^\top]$ has bounded maximum sparse eigenvalue, i.e., 
%     $
% \phi_{\max}(Cs^*, \Sigma_i)
%         \leq \phi_u   < \infty,
%     $
%     % \begin{align*}
%     %     0< \phi_\ell &\leq \phi_{\min}(C s^*, \Sigma_i) \leq \phi_{\max}(Cs^*, \Sigma_i)
%     %     \leq \phi_u   < \infty
%     % \end{align*}
%     for all $i \in [K]$,
%      where $C$ is the same constant as in part (c).
% \end{enumerate}
% \end{assumption}

% \begin{assumption}[Assumptions on the true parameter]
% \label{assumptions: arm-separation}
% We assume the followings:
% \vspace{-5pt}
% \begin{enumerate}[label = (\alph*),leftmargin=*]
% \itemsep0em
%     \item \label{item: beta-l1} \textit{Sparsity and soft-sparsity:} $\norm{\beta^*}_0 = s^*$ and $\norm{\beta^*}_1 \leq \bmax$ for constants $s^*\in\bbN, \bmax\in\bbR_+$.
%     \item \label{item: margin-cond} \textit{Margin condition:} There exists positive constants $\Delta_*, A$ and $\alpha\in [0, \infty)$, such that for $h \in \left[ A \sqrt{\log(d)/T}, \Delta_*\right]$ and for all $t\in [T]$,
%    $\pr\left( x_{a^*_t}(t)^\top \beta^* \leq \max_{i \neq a^*_t} x_{i}(t)^\top \beta^* +h\right) \leq  \left(\frac{h}{\Delta^*}\right)^\alpha.$
% \end{enumerate}
% \end{assumption}

% \begin{assumption}[Assumption on Noise]\label{assumptions: noise}
% We assume that the random variables $\{\epsilon(t)\}_{t\in[T]}$ are independent and also independent of the other processes and each one is $\sigma-$Sub-Gaussian, i.e.,  $\bbE [e^{a \epsilon(t)}] \leq e^{\sigma^2 a^2/2}$  for all $ t \in [T]$ and $a\in \bbR$. 
% \end{assumption}

% \textit{Remarks:} In assumption \ref{assumptions: contexts}\ref{item: context_subgaussian}, $\norm{X}_{\psi_2}:= \sup_{u: \norm{u}_2\le 1} \norm{u^\top X}_{\psi_2}$ is the Orlicz-norm, where for a random-variable $Z$,  $\norm{Z}_{\psi_2} :=\inf \{\lambda >0 : \bbE \exp(Z^2/\lambda^2) \leq 2\}$. It states that the context distribution for each arm is sub-Gaussian, this assumption does not require the distributions to have zero mean. We remark that while we assume i.i.d. contexts across time, for each time $t$, the contexts across different arms are allowed to be correlated. The zero-mean sub-Gaussian assumption on the noise \ref{assumptions: noise} is satisfied by various families of distributions, including normal distribution and bounded distributions, which are commonly chosen noise distributions. The margin condition \ref{assumptions: arm-separation}\ref{item: margin-cond} essentially controls the hardness of the bandit instance, with $\alpha=\infty$ making it easiest due to a deterministic gap between arms, and $\alpha=0$ making it hardest (no a-priori information about arm separation). A more detailed discussion about the assumptions is provided in the Appendix \ref{app: assumptions discussion}.


\section{LOWER BOUNDS ON REGRET}\label{sec: lower bound}
The first question that we want to address is what is the inherent cost of privacy in SLCB. Hence, we derive a minimax regret lower bound on the regret achieved by any algorithm ensuring $(\epsilon,\delta)$-JDP for SLCB. The other goal is to understand the cost of privacy on the minimax lower bound compared to the existing lower bounds for SLCB without differential privacy. First, we formally define the minimax regret in this setting. 
\begin{definition}[Minimax regret] We define the minimax regret in the $(\epsilon,\delta)$-JDP SLCB  as $R^{\mathrm{minimax}}_{(\epsilon,\delta)}(T) := \inf_{\pi\in \Pi(\epsilon,\delta)} \sup_{P_{\bX,\br}\in \cB} \bbE[R_{\pi}(T)]$, where the supremum is taken over $\cB$, i.e. the space of SLCB instances, and the infimum is taken over $\Pi(\epsilon,\delta)$, i.e. the space of $(\epsilon,\delta)$-JDP policies. 
\end{definition}
% The expectation in the above definition is with respect to the interaction between the policy $\pi$ and the bandit environment $P_{X,Y}$. The minimax regret is defined over bandit instances satisfying just the boundedness assumption for the contexts (to make the lower bound context scale free), the margin condition (to capture the effect of $\alpha$, which controls the hardness of the bandit instance) and the sub-Gaussian noise (to control the tail behavior of the rewards). 
Further details about the minimax regret, the space of bandit instances and the associated probability space are in Appendix \ref{app: lower bound proof new}.
Our first result gives a lower bound on the minimax regret, in terms of the impact of the bandit model parameters $s^{*}, d, T$, and privacy parameters $\epsilon, \delta$.

\begin{theorem}[Lower Bound]\label{thm:lb_edp}
    If $\epsilon, \delta> 0$ and $\epsilon^{2} < \log(1/\delta)$, then for sufficiently large $s^* \log(d/s^*)$ the minimax regret for SLCBs under $(\epsilon,\delta)$-JDP
    % \small{\begin{align*}
    % R^{\mathrm{minimax}}_{(\epsilon,\delta)}(T) = ~\Omega\Big( \max &\{\underbrace{ \log (d/s^*) \sqrt{s^*}\left\{\epsilon^2/\log(1/\delta)\right\}^{-1/2}}_{\text{private and high-d}},\\
    % &\underbrace{\sqrt{s^* T \log (d/s^*)}}_{\text{non-private and high-d}}\}\Big)\,.
    \begin{align*}
        & R^{\mathrm{minimax}}_{(\epsilon,\delta)}(T)=\\
        &\Omega\Big(\max \Big\{\underbrace{  \sqrt{\frac{s^* \log^2 (d/s^*) \log(1/\delta)}{\epsilon^2}}}_{{\text{private} \text{and high-d}}}, \underbrace{\sqrt{s^* T \log (d/s^*)}}_{\substack{\text{non-private}\\ \text{and high-d}}}\Big\}\Big).
    \end{align*}
    %\geq  \max \left\{\underbrace{C_{zcdp}(\log d)^{\frac{1+\alpha}{2}} \rho^{-\frac{1+\alpha}{2}}}_{\text{private and high-d}}, \underbrace{C_{no-dp}(\log d)^{\frac{\alpha+1}{2}} T^{\frac{1-\alpha}{2}}}_{\text{non-private and high-d}}, \underbrace{\log T}_{\text{non-private and low-d}} \right\}.
    % \end{align*}} % where $C', C''$ are constants independent of $d, T, \epsilon, \delta, \alpha$.
    Additionally, for $\delta=0$, we get $R^{\mathrm{minimax}}_{\epsilon}(T) = \Omega\Big(\max \{s^{*} \log^{3/2} (d/s^*) \epsilon^{-1}, 
    {\sqrt{s^* T\log (d/s^*)} }\rbrace\Big).$
\end{theorem}
% The constants in the above theorem depend on other parameters such as $\xmax$ (arising from assumption \ref{assumptions: contexts}\ref{item: context_bound}) and $\sigma$ (from assumption \ref{assumptions: noise}), which we treat as constants in this work. 
\textit{Implications.} (i) This is the first lower bound for SLCBs with JDP. All the existing bounds with JDP are for low-dimensional LCBs with JDP. (ii) Theorem~\ref{thm:lb_edp} indicates that the impact of privacy appears in the regret lower bound when { $\epsilon^2/\log (1/\delta) < \log (d/s^*)/T$}. For $\delta = 0$, the above theorem also states that the cost of privacy becomes prevalent in the regime { $\epsilon < \sqrt{s^*} \log(d/s^*)/\sqrt{T}$}, which matches in spirit with the lower bound of~\citep{azize2022privacy_dpband} for a fixed low-dimensional context set, where the impact of privacy appears for $\epsilon < T^{-1/2}$. Additionally, in SLCB, the dimension also matters for the transition. This phenomenon is also reflected in our regret upper bounds. 

\textit{Proof Technique.} Our proof differs from the existing lower bound techniques for private bandits in \citep{shariff2018differentially,basu2019differential_dpband,azize2022privacy,azize2023privacy}, and non-private SLCB setting \citep{li2021regret}.
% Here, we cannot use the generic lower bound proving technique of~\cite{azize2023privacy} as it works for a fixed context set and a fixed set of arms available at every step. In our setting, the contexts are randomly generated at every step. To tackle this, \cite{li2021regret} proposed another proof technique. We cannot use it as it requires deploying the Bayes optimal policy over generated contexts at an intermediate step. But Bayes optimal policy does not satisfy the $(\epsilon, \delta)$-JDP constraints, and thus, cannot be used. 
Rather our proof depends on converting the regret lower bound problem to an estimation lower bound problem following \cite{he2022reduction}, and combing the information-theoretic techniques for sparse linear models~\citep{duchi2013distance} and { privacy-restricted lower bound techniques in~\citep{azize2023privacy, kamath2022improved}.} 

% We show that given this space, we can reduce the regret problem in SLCBs to an estimation problem without using the non-private Bayes optimal policy. Then, we deploy a continuous Fano's inequality to lower bound the estimation error for $\beta^*$ at any $t$. This encapsulates the geometric nature of sparse linear space of $\beta^*$ and its estimates. Followed by this, we leverage the data processing inequality for $(\epsilon, \delta)$-DP bandit policies~\citep{azize2023privacy}. It brings in the limit of information generated by $(\epsilon, \delta)$-JDP policies to yield an estimate of $\beta^*$. Together they lead to our proposed lower bound.

% \textit{Proof sketch.} The detailed proof is given in Appendix \ref{app: lower bound proof}. First, we prove a lower bound for $\rho-$zCDP policies. In the proof, we construct hard-bandit instances satisfying the requirements in $\cP_\alpha$ and carefully control the KL-divergence terms with a KL-decomposition specific to contextual bandits and $\rho$-zCDP. We know that an algorithm satisfying $\rho-$zCDP achieves $(\epsilon,\delta)$-DP, with $\rho\approx \epsilon^2 / 2\log(1/\delta)$ \citep[Lemma 3.5]{Bun:tCDP} for a given $\delta > 0$, which allows us to further establish the minimax regret lower bound for $(\epsilon,\delta)$-JDP setting.



\section{REFINED ANALYSIS: PEELING FOR $(\epsilon,\delta)$-DP ERM}\label{section: general result}
In this section, we describe and analyze an $(\epsilon,\delta)$-DP algorithm, which can be used for general private empirical risk minimization. While the algorithm appears in \citep{cai2021cost} in sparse regression setting, we present a refined and simpler proof of the utility guarantee such that the results are applicable not only in the standard regression setting with independence across observations, but also to data arising from highly dependent and dynamic bandit environments. 

The well-known \emph{Peeling} algorithm (Appendix~\ref{section: background_privacy}) is used for $(\epsilon, \delta)$-DP top-$s$ selection problem~\citep{dwork2021differentially}.
We denote the output of Peeling applied to a vector $v \in \bbR^d$ as $\cP_s(v ;\epsilon,\delta, \lambda)$, where $\epsilon, \delta$ are privacy parameters and $\lambda$ is the scale parameter of the Laplace noise. For $v\in \bbR^d$, and an index set $S\subseteq[d]$, $v_S\in\bbR^d$ denotes the vector such that $v_S$ matches $v$ on indices in $S$ and is 0, elsewhere. 
Peeling returns a $s$-sparse vector in $\bbR^d$.  It is important to point out that the peeling algorithm is an important building block of N-IHT, which in turn is a crucial component of FLIPHAT. 
% Therefore, our algorithm does not suffer from the curse of dimensionality, i.e., it enjoys a poly-logarithmic dependence in the ambient dimension $d$. 

\textbf{A Generic Analysis of N-IHT.} Let us consider $n$ observations $(x_1,y_1),\dots,(x_n,y_n)$, 
where $x_i\in \bbR^d$ and $y_i\in\bbR$ for all $i\in[n]$, arising from a joint distribution $\cQ$. We denote the design matrix by $X$ and $y\in\bbR^n$ as the vector of responses. We note that we neither assume any particular model (e.g. linear model), nor independence across observations. Now, we wish to use Algorithm \ref{alg:noisy-IHT} to minimize the empirical risk
$\cL(\theta|X,y) := \frac{1}{n}\sum_{i=1}^n \ell((y_i, x_i);\theta)$ w.r.t. a loss function $\ell(\cdot; \cdot)$.
% The usual regression setting uses the squared error loss $\ell(y_i, x_i;\theta) = (y_i - x_i^\top\theta)^2$ and the linear model $y_i=x_i^\top\theta^*+\xi_i$ for some true parameter $\theta^*$ and i.i.d. error terms $\xi_i$. 
In Algorithm~\ref{alg:noisy-IHT}, $\clip_R(z) := z\min \{1, R/|z|\}$ and $\clip_R$ on a vector $y$ means a coordinate-wise application (Line 3). $\cP_s$ is the peeling subroutine serving as a private hard thresholding step (Line 4). Finally, $\Pi_C$ is the (Euclidean) projection on the ball $\{v\in\bbR^d\mid \norm{v}_1\leq C\}$, i.e., $\Pi_C(x) = \argmin_{v: \norm{v}_1 \le C} \norm{x -v}_2$ (Line 5).
We note that the clip function and the projection step at the end are crucial for the sensitivity analysis to get a DP guarantee for the entire algorithm. For subsequent reference, we denote N-IHT$(X,y|s,\epsilon,\delta, M, R, B, \eta, C)$ to be the output of Algorithm \ref{alg:noisy-IHT} on data $(X,y)$ with the tuning parameters as mentioned in Algorithm \ref{alg:noisy-IHT}.


Assume that $\norm{x_i}_{\infty}\leq \xmax$ and $\theta^*\in\bbR^d$ is any point such that  $\norm{\theta^*}_1\leq \bmax$ and $\norm{\theta^*}_0=s^*$. Now, we consider three \textit{good} events. First, we define the event $\cE_1$ as the one satisfying the infimum of minimum sparse eigenvalue, i.e. $\inf_{\theta} \phi_{\min}(Cs^*, \nabla^2 \cL(\theta)) \geq \underline{\kappa}$, and the supremum of maximum sparse eigenvalue, i.e. $\sup_{\theta} \phi_{\max}(Cs^*, \nabla^2 \cL(\theta)) \leq \bar{\kappa}$ (ref. Definition~\ref{def: sparse eigen value}). Here, $\nabla^2 \cL$ is the Hessian computed for the data $(X,\clip_R(y))$. Second, $\cE_2 := \left\{\norm{\nabla \cL(\theta^*)}_{\infty} \leq \bar{g}\right\}$, where $\nabla \cL$ is the corresponding gradient. Finally, $\cE_3 := \left\{\max_{m\in[M]} \bW_m \leq \bar{W}_{(\epsilon,\delta)}\right\}.$
Here, $\bW_m :=\sum_{i\in[s]} \Vert\bw_i^{(m)}\Vert_{\infty}^2 + \Vert\tilde{\bw}_{S^m}^{(m)}\Vert_2^2$ is the total amount of noise injected in the $m$-th iteration, where $\bw_i$ and $\tilde{\bw}$ are the two sources of noise introduced by Peeling $\cP_s$ in Algorithm~\ref{alg: peeling}.
With these events, we derive an upper bound on the $\ell_2$ distance of $\hat{\theta}$, i.e. the output of Algorithm~\ref{alg:noisy-IHT}, from $\theta^*$.

\setlength{\textfloatsep}{6pt}
\begin{algorithm}[t!]
% \small
\caption{N-IHT}\label{alg:noisy-IHT}
 % \small
\begin{algorithmic}[1]
\REQUIRE Data $\bX, \by$, sparsity $s$, privacy level $\epsilon, \delta$, number of iterations $M$, truncation level $R$, noise scale $B$, step-size $\eta$, projection level $C$

\STATE Initialize $\theta^0 \in \bbR^d$.

\FOR{$m = 0, 1, \dots, M-1$}
    \STATE $\theta^{m+0.5} = \theta^m - \eta\nabla \cL(\theta^{m}|X, \clip_R(y))$ 
    \STATE $\tilde{\theta}^{m+1} = \cP_s(\theta^{m+0.5};\epsilon/M, \delta/M,\eta B / n)$. 
    \STATE $\theta^{m+1} = \Pi_C(\tilde{\theta}^{m+1})$.
\ENDFOR

\RETURN \textbf{Return} $\hat{\theta}=\theta^{M}$
\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{thm: general result}
     Let $\eta=1/2\bar{\kappa}, M\ge 28\kappa\log(\bmax^2 n)$, $C\ge \norm{\theta^*}_1$ and $s \gtrsim \kappa^2 s^*$. Then, with probability at least $1-\Pr(\cE_1^c)-\Pr(\cE_2^c)-\Pr(\cE_3^c)$, %we have
    $$\norm{\theta^M - \theta^*}_2^2\leq \frac{1}{n} + C_1\kappa^2\bar{W}_{(\epsilon,\delta)} + C_2 \frac{\kappa^2}{\underline{\kappa}^2} (s+s^*) \bar{g}^2,$$
    for suitably large constants $C_1, C_2>0$, where the probability measure $\Pr$ is that arising from the joint distribution $\cQ$ and the randomness due to privacy. $\kappa=\bar{\kappa}/\underline{\kappa}$ denotes the condition number of the Hessian of loss $\cL$.
\end{theorem}\vspace*{-.5em}
The proof is detailed in Appendix~\ref{app: proof of general result}. For the squared error loss $\ell((y,x);\theta)=(y-x^\top\theta)^2$ and independent samples, the output of Algorithm~\ref{alg:noisy-IHT} with $B=R+\xmax\bmax$ is $(\epsilon,\delta)$-DP~\citep{cai2021cost}. 
In other cases, one can tune $B$ depending on the sensitivity requirement to obtain DP guarantees.
% On a different note, if the choice of $R$ is made such that $\{\clip_R(y)=y\}$ occurs with high probability, then we can replace the gradient and Hessian terms in the good events by corresponding terms with respect to the data $(X,y)$ instead of $(X,\clip(y))$ at the cost of a reduction in the probability due to $\cE_4$.

\textit{Generic Implications.} The theorem is general in the sense that it holds for $(X,y)$ arising from any joint distribution $\cQ$ and $\ell(\cdot; \cdot)$ being any loss function. The Laplace noise (in Peeling) is not mandatory to use this result. The first term in the upper bound goes to $0$ as the sample size increases. The third term, controlled by the behavior of the gradient of the loss at the target point, typically is the statistical bound. The second term is the cost we pay for ensuring $(\epsilon,\delta)$-DP for the output. Clearly, we should not expect $\norm{\theta^M-\theta^*}_2$ to go to 0, for arbitrary $\theta^*$. However, once we make certain assumptions about the model (e.g., linear model where $\theta^*$ is the true data generating parameter), and the loss structure (e.g., squared error), the result would allow us to `plug-in' standard guarantees about control of the good events in this result and obtain specific estimation bounds. 

% \paragraph{Standard sparse regression setting:} For the independent observations case with squared error loss $\ell(y,x;\theta)=(y-x^\top\theta)^2$ and linear model, we have $\nabla^2 \cL(\theta) = X X^\top/n$ (free of $\theta$) and thus, under typical assumptions (well-behaved covariance matrix $\Sigma$ for each $x_i$), we can ensure that $\cE_1$ occurs with high probability. The clipping constant $R$ enters the bound through the terms $\bar{W}$ and $\bar{g}$. The former (for Laplace noise with the appropriate scale as mentioned) can be taken as a suitable constant multiple of $R^2 (s^* \log d)^2 \log(\log n/\delta)\log^2 n/(n^2\epsilon^2)$ to ensure that $\cE_3$ occurs with high probability. We note that had we replaced the Laplace noise by Gaussian (the scale needs to be revisited to ensure correct privacy guarantee), the theorem still remains valid - with a potential change in the order of the terms in $\bar{W}$. The gradient term $\bar{g}$ can be made free of $R$, by conditioning on the high-probability event $\cE_4 = \{\clip_R(y_i) = y_i \quad \forall i\in[n]\}$, taking $R=\xmax\bmax+\sigma\sqrt{2\log n}$, where $\sigma$ is the sub-Gaussian parameter for the errors $\xi$. Finally, for this loss (under $\cE_4$), $\nabla \cL (\theta^*) = X^\top \xi / n$, where $\xi\in\bbR^n$ is the vector of i.i.d. sub-Gaussian$(\sigma)$ errors and hence $\bar{g}$ can be chosen as $2\sigma\xmax\sqrt{\log d/n}$. Plugging these into the result, we can get an estimation guarantee for this problem.
 
 % \paragraph{LCB:}
 % From our analysis, it is clear that if we can only show similar control on the events $\cE_1$ and $\cE_3$, then the result would follow. Control on the good events in the linear bandit setting is discussed in Appendix \ref{app: bandit corollary} and constitute an important part of the regret analysis for FLIPHAT. 
 
 % In the following section, we use N-IHT as a building block for our proposed algorithm and demonstrate that the current theorem can be utilized to establish the upper bound for the regret.
 
 % For the set $\cE_1$, we can use Proposition B.5 \cite{chakraborty2023thompson} and for $\cE_2$, we can use Proposition 3 \cite{chakraborty2023thompson}. We note that control on $\cE_3$ stays the same owing to the same peeling mechanism being used. 

\vspace*{-.3em}\section{FLIPHAT: ALGORITHM DESIGN \& REGRET ANALYSIS}\label{sec: upper bound}\vspace*{-.3em}
In this section, we propose a novel algorithm FLIPHAT for the SLCB setting, which is guaranteed to be $(\epsilon,\delta)$-JDP. 
Then, we derive an upper bound on its expected regret that matches the regret lower bound from Section~\ref{sec: lower bound} up to logarithmic terms.

\vspace*{-.2em}\subsection{Algorithm Design}\vspace*{-.2em}

We present the pseudocode of FLIPHAT in Algorithm \ref{alg: fliphat}. FLIPHAT has three components. 

\textit{First}, we employ the doubling trick~\citep{besson2018doubling}, i.e. dividing the entire time horizon into episodes of geometrically progressive lengths. Specifically, the $\ell-$th episode begins at step $t_{\ell}=2^{\ell}$. At the beginning of each episode, the underlying algorithm restarts, computes the required estimates, and the episode continues for $N_\ell = 2^{\ell+1} - 2^{\ell} = 2^{\ell}$ steps. In non-private bandit, we use doubling trick to make the algorithm `anytime', but for private bandits, it also helps to reduce the number of times for which we have to calculate any private estimates from the data. Since DP is typically achieved by adding scaled Laplace noise with the newly computed estimates~\citep{dwork2014algorithmic}, doubling ensures that we do not add noise for more than a logarithmic number of times. This is important for regret optimality.


% the added Laplace noise has to scale with the \textit{sensitivity} of the computed estimates, i.e. how much it can change if an observation changes. Typically, the scale grows linearly with the number of samples used for estimation. 
\textit{Second}, to ensure DP, we use the \textit{forgetfulness} technique, i.e. at the beginning of an episode, we only use the data collected from the previous episode to generate the estimate. In the current episode, we do not update the estimate further. This \textit{forgetful} strategy (the observed data from an episode is used just once at the start of the next episode and then forgotten) allows us to guarantee that the overall algorithm is private, if the computed estimates are private. 
The main idea is that a change in a reward and context will only affect the estimate calculated in one episode. This allows parallel composition of DP and stops the aggravated accumulation of Laplace noise over time, yielding better regret guarantees.

\textit{Third}, we use N-IHT (Algorithm \ref{alg:noisy-IHT}) as the private sparse linear regression oracle to estimate the linear parameter from the observed samples. 
At the beginning of $(\ell+1)$-th episode (line 8), we feed N-IHT the data $(X_\ell,y_\ell)$ consisting of the chosen contexts and observed rewards from the $\ell$th episode (line 13). Other tuning parameters $(s,\epsilon,\delta,\eta,C)$ are not explicitly mentioned as they stay same for all $\ell$'s. 

\begin{algorithm}[t!]
% \small
\caption{FLIPHAT}\label{alg: fliphat}
 % \small
\begin{algorithmic}[1]
\REQUIRE Sparsity $s$, privacy level $\epsilon, \delta$, step-size $\eta$, projection level $C$, sequence of iteration lengths $\{M_\ell\}$, truncation levels $R_\ell$

\FOR{$\ell=0$:} 
    \STATE Play a random arm $a_1\in[K]$ \STATE Observe $r(1) = x_{a_1}(1)^\top \beta^*+\epsilon(1)$. 
    \STATE Set $X_0=\{x_{a_1}(1)\}$, $y_0=\{r(1)\}$.
\ENDFOR
\FOR{$\ell=1,2,\dots$}
    \STATE Set $B=R_\ell+\xmax\bmax$
    \STATE Estimate $\hat{\beta}_\ell = \text{N-IHT}^*(X_{\ell-1}, y_{\ell-1}|M_\ell, R_\ell, B)$
    \STATE Set $X_\ell = \{\}, y_\ell = \{\}$
    \FOR{$t=t_{\ell}, t_{\ell}+1,\dots, t_{\ell+1}-1$}
        \STATE Play $a_t = \argmax_a x_{a}(t)^\top \hat{\beta}_\ell$
        \STATE Observe reward $r(t) = x_{a_t}(t)^\top\beta^* + \epsilon(t)$
        \STATE Store $X_\ell=X_\ell \cup \{x_{a_t}(t)\}$, $y_{\ell}=y_{\ell}\cup\{r(t)\}$
    \ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

% We now describe FLIPHAT (Algorithm \ref{alg: fliphat}) in detail. Firstly, note that $\text{N-IHT}$ refers to , . Here, $\ell=0,1,\dots$ indexes the episodes with $t_{\ell}=2^{\ell}$ marking the beginning of the $\ell-$th episode. Thus, episode $\ell$ has length $N_\ell = 2^{\ell+1} - 2^{\ell} = 2^{\ell}$. In the $\ell-$th episode, we only estimate $\beta$ once at time $t=t_\ell$ (start of that episode) using $N_{\ell-1}$ data points (from the previous episode) and then use this estimate, $\hat{\beta}_\ell$ throughout the episode. 
% % The first episode $(\ell=0)$ has only $1$ time point and it starts with a random initialization $\hat{\beta}_0$. Then $X_0 = \{x_{a_1}(1)\}, y_0 = \{r(1)\}$ is used as the input of N-IHT (with the chosen tuning parameters) and we obtain $\hat{\beta}_1$, which is then used consistently for $t=2,3$ (only two time points in episode $\ell=1$) and so on. 
% The forgetting trick along with the privacy guarantee for N-IHT gives us the following JDP property of FLIPHAT.
\begin{theorem}
    \label{thm: fliphat DP}
    FLIPHAT preserves $(\epsilon, \delta)$-JDP.
\end{theorem}
To this end, we point out that FLIPHAT also enjoys the reward-DP \citep{hanna2024differentially}, where the algorithm only ensures the privacy protection of the reward stream. 
In this setup, the adversary is only allowed to perturb the reward stream which is quite a strong restriction on the nature of the adversary. JDP protects against a more general adversary and protects the information in both rewards and contexts. %This is important for applications where context is a user data, e.g. personalized medicine.
\subsection{Regret Analysis}
Now, we present the regret upper bound of FLIPHAT. 
We first briefly discuss the assumptions that we impose on the various model components, which are well accepted in the literature on SLCB~\citep{zhang2008sparsity, zhang2010nearly, bastani2020online, li2021regret, chakraborty2023thompson}. \textit{In regret analysis, we do not require any additional assumption for privacy.}%, apart from only those required for SLCB.} 

% \begin{definition}[Sparse Riesz Condition]
% \label{def: sparse eigen value}
% For a $d\times d$ positive semi-definite matrix $A$, its maximum and minimum sparse eigenvalues with parameter $s\in [d]$ are defined as $\phi_{\min}(s; A):= \inf_{u: u \neq 0, \norm{u}_0 \leq s} u^\top A u /\norm{u}_2^2, \quad \phi_{\max}(s; A) := \sup_{u: u \neq 0, \norm{u}_0 \leq s} u^\top A u/\norm{u}_2^2$.
% % We say $A$ has Sparse Riesz Condition if  $0< \phi_{\min}(s, A) \leq \phi_{\max}(s; A) < \infty$.
% \end{definition}

\begin{assumption}[Assumptions on Context Distributions] \label{assumptions: contexts}
We assume that
\begin{enumerate}[label=(\alph*),leftmargin=*,nosep]
\itemsep0em
    \item \label{item: context_bound} \textit{Boundedness:} $\bbP_{x\sim P_i} (\norm{x}_\infty \leq \xmax) =1$ for all $i\in[K]$ for a constant $\xmax\in \bbR^+$.
    \item \label{item: context_subgaussian} \textit{Bounded Orlicz norm:} For all arms $i \in [K]$ the distribution $P_i$ is bounded in the Orlicz norm, i.e., $\norm{X}_{\psi_2}\leq \vartheta$ for $X\sim P_i$ for all $i\in [K]$. %\sapta{may use new line for equation}
    \item \label{item: anti-concentration} \textit{Anti-concentration:} There exists a  constant $\xi\in \bbR^+$ such that for each $u\in \{v\in\bbR^d : \norm{v}_0 \leq Cs^*, \norm{v}_2=1\}$ and $h\in \bbR^+$ 
    $P_i(\innerprod{x, u}^2 \leq h) \leq \xi h,$
    for all $i\in [K]$, ,where $C\in (2,\infty)$.
    \item \label{item: sparse_eigenvalue} \textit{Sparsity:} The matrix $\Sigma_i := \bbE_{x\sim P_i} [x x^\top]$ has bounded maximum sparse eigenvalue, i.e., 
    $
\phi_{\max}(Cs^*, \Sigma_i)
        \leq \phi_u   < \infty,
    $
    % \begin{align*}
    %     0< \phi_\ell &\leq \phi_{\min}(C s^*, \Sigma_i) \leq \phi_{\max}(Cs^*, \Sigma_i)
    %     \leq \phi_u   < \infty
    % \end{align*}
    for all $i \in [K]$,
     where $C$ is the same constant as in part (c).
\end{enumerate}
\end{assumption}

\begin{assumption}[Assumptions on the true parameter]
\label{assumptions: arm-separation}
We assume the following:
\vspace{-5pt}
\begin{enumerate}[label = (\alph*),leftmargin=*,nosep]
\itemsep0em
    \item \label{item: beta-l1} \textit{Sparsity and soft-sparsity:} $\norm{\beta^*}_0 = s^*$ and $\norm{\beta^*}_1 \leq \bmax$ for constants $s^*\in\bbN, \bmax\in\bbR_+$.
    \item \label{item: margin-cond} \textit{Margin condition:} There exists positive constants $\Delta_*, A$ and $\alpha\in [0, \infty)$, such that for $h \in \left[ A \sqrt{\log(d)/T}, \Delta_*\right]$ and $\forall t\in [T]$, $\pr\left( x_{a^*_t}(t)^\top \beta^* \leq \max_{i \neq a^*_t} x_{i}(t)^\top \beta^* +h\right) \leq  \left(\frac{h}{\Delta^*}\right)^\alpha$
\end{enumerate}
\end{assumption}
\begin{assumption}[Assumption on Noise]\label{assumptions: noise}
We assume that the random variables $\{\epsilon(t)\}_{t\in[T]}$ are independent and also independent of the other processes and each one is $\sigma-$Sub-Gaussian, i.e.,  $\bbE [e^{a \epsilon(t)}] \leq e^{\sigma^2 a^2/2}$  for all $ t \in [T]$ and $a\in \bbR$. \vspace*{-.5em}
\end{assumption}

\textit{Remarks:} In ~\ref{assumptions: contexts}\ref{item: context_subgaussian}, $\norm{X}_{\psi_2}:= \sup_{u: \norm{u}_2\le 1} \norm{u^\top X}_{\psi_2}$ is the Orlicz-norm, where for a random-variable $Z$,  $\norm{Z}_{\psi_2} :=\inf \{\lambda >0 : \bbE \exp(Z^2/\lambda^2) \leq 2\}$. It states that the context distribution for each arm is sub-Gaussian, this assumption does not require the distributions to have zero mean. We remark that while we assume i.i.d. contexts across time, for each time $t$, the contexts across different arms are allowed to be correlated. The zero-mean sub-Gaussian assumption on the noise (Assumption~\ref{assumptions: noise}) is satisfied by various families of distributions, including normal distribution and bounded distributions, which are commonly chosen noise distributions. The margin condition (Assumption~\ref{assumptions: arm-separation}\ref{item: margin-cond}) essentially controls the hardness of the bandit instance, with $\alpha=\infty$ making it easiest due to a deterministic gap between arms, and $\alpha=0$ making it hardest, i.e. no apriori information about arm separation. A detailed discussion on the assumptions is in Appendix~\ref{app: assumptions discussion}.

Next, we derive a bound on estimation error of the parameter $\beta^*$ at any episode $\ell$, which is central to the regret analysis and a consequence of Theorem~\ref{thm: general result}. Note that $(X_\ell, y_\ell)$ are only conditionally i.i.d., and not marginally independent. %which is proved in Appendix \ref{app: proof of general result}. %The proof is essentially obtaining control on the good events as required in Theorem \ref{thm: general result}. 

\begin{proposition}[Estimation Control for Episode $\ell$]\label{prop: estimation episode}
    Suppose Assumptions \ref{assumptions: contexts}, \ref{assumptions: arm-separation}(a) and \ref{assumptions: noise} holds. If we set $\eta=1/2\bar{\kappa}, C=\bmax, s\gtrsim \kappa^2s^*, M_{\ell+1} = 28\kappa \log (\bmax^2 N_\ell)$ and $R=\xmax\bmax+\sigma\sqrt{2\log N_\ell}$, we have for all $\ell>1$
    \begin{equation}
        \Vert\hat{\beta}_{\ell+1} - \beta^*\Vert_2^2 \lesssim  \Lambda_{\textsc{non-private}} + \Lambda_{\textsc{private}}
    \end{equation}
    with probability at least $1-c_1\exp(-c_2 \log d) - \Pr(\cE_{1\ell}^c) - 1/N_\ell$, where $\Lambda_{\textsc{non-private}} = \sigma^2\kappa^2 \frac{(s + s^*)\log d}{\underline{\kappa}^2 N_\ell}$, and  $\Lambda_{\textsc{private}} = \sigma^2\kappa^2 \frac{(s\log d)^2\log\left( \frac{\log N_\ell}{\delta}\right)\log^3 N_\ell}{N_\ell^2\epsilon^2}$ 
    are the non-private (statistical) and private terms in the estimation bound. Here,  $\cE_{1\ell}=\{\underline{\kappa}\leq \phi_{\min}(Cs^*, \hat{\Sigma}_\ell)<\phi_{\max}(C s^*, \hat{\Sigma}_\ell) \leq \bar{\kappa}\}$, $\kappa=\bar{\kappa}/\underline{\kappa}$, and $\hat{\Sigma}_\ell = X_{\ell} X_{\ell}^\top / N_{\ell}$ is the covariance of the contexts observed in $\ell$-th episode.
\end{proposition}\vspace*{-.5em}

% Proposition B.5 \cite{chakraborty2023thompson} shows that with $\bar{\kappa}\asymp \log K, \underline{\kappa}\asymp 1/K$, we have
% $$\Pr(\cE_{1\ell}^c)\lesssim \exp(c_3 s^*\log (c_4 d) - c_4 N_\ell)$$
% where the constants $c_3,c_4,c_5$ could depend on $K < d$.  Essentially, this ensures that sufficient choice of $N_\ell \gtrsim s^*\log d$ (i.e., $\ell \gtrsim \log(s^*\log d)$) would allow us to control the regret suffered for these later episodes, which allows us to derive the regret guarantee for FLIPHAT presented below. {  delete this}

Proposition B.5 of \citep{chakraborty2023thompson} allows us to control the term $\bbP(\cE_{1\ell}^c)$ appearing in the above proposition, which is used to derive the regret guarantee for FLIPHAT, as presented below.
\begin{theorem}[Regret bounds for FLIPHAT]\label{thm: regret}
    Suppose Assumption \ref{assumptions: contexts}, \ref{assumptions: arm-separation}, and \ref{assumptions: noise} hold. Then for any privacy level $\epsilon>0$ and $\delta < e^{-1}$, and with the same choices of the tuning parameters as in Proposition \ref{prop: estimation episode} with $\bar{\kappa} \asymp  \log K$ and $\underline{\kappa} \asymp K^{-1}$, FLIPHAT enjoys the following regret bound 
    \[
    \bbE[R(T)] \lesssim  \xmax \bmax(s + s^*) \log d + I_\alpha \vee J_\alpha(\epsilon, \delta),
    \]\vspace*{-.5em}
    where 
    \begin{align*}\vspace*{-.1em}
    &I_\alpha = 
    \begin{cases}
        \frac{1}{\Delta_*^\alpha}\left(\frac{T^{\frac{1-\alpha}{2} - 1}}{1-\alpha}\right)\{(s + s^*)^2 \log d\}^{\frac{1+\alpha}{2}}, & \alpha \in [0, \infty) \\%&\alpha\in[0,\infty) \\  
         (s + s^*)^2 \log d , & \alpha = \infty. \\% & \alpha = \infty,
    \end{cases}\\
    % \end{align*}
    % and 
    % \begin{align*}
    &J_\alpha(\epsilon, \delta) = \begin{cases}
        \Psi_\alpha(T)\left\{\frac{(s + s^*)^3\log^2 d \log(1/\delta)}{\epsilon^2}\right\}^{\frac{1+\alpha}{2}}, & \alpha \in [0, \infty)\\
        \frac{(s + s^*)^3 \log^2 d \log(1/\delta)}{\epsilon^2}, & \alpha = \infty.       
    \end{cases}
    \end{align*}
    Here, $\Psi_{\alpha}(T) = \frac{1}{\Delta_*^\alpha}\sum\limits_{n=0}^{\floor{\log T}+1} \frac{n^{2\alpha+2}}{2^{n\alpha}}$.
For $\alpha > 0$, $\Psi_{\alpha}(T) \lesssim \frac{\Gamma(3+2\alpha)}{\Delta_*^{\alpha} (\alpha \log 2)^{3+2\alpha}}$, and $\Psi_{0}(T) \lesssim {\log^3 T}$.\vspace*{-.5em}
\end{theorem}
The first term in the upper bound $\xmax\bmax s^*\log d$ is intuitively the unavoidable part of regret, that is incurred during the initial part of the horizon when $\beta^*$ has not been estimated well enough. The second term is essentially two terms - $I_\alpha$ is the non-private statistical part of the regret while $J_\alpha(\epsilon,\delta)$ is the part arising due to the privacy constraint.
% We note that both the terms depend on $\alpha$, which we recall as the margin parameter in Assumption \ref{assumptions: arm-separation}. 
The non-private term $I_\alpha$ is similar to the corresponding term in the regret bound for SLCB in \citep{chakraborty2023thompson, li2021regret}. Furthermore, for $\alpha = 0$, the upper bound in Theorem \ref{thm: regret} matches with the problem-independent lower bound in Theorem \ref{thm:lb_edp} in terms of time horizon $T$ (up to logarithmic factors), context dimension $d$ and privacy parameters $\epsilon,\delta$.
Below, we state the implications.

% \textbf{Proof Sketch.} The main technical challenge of the proof lies in the analysis of online private IHT (Proposition \ref{prop: estimation episode}). It has two main steps. (i) Under the restricted convexity and restricted smoothness assumptions, we establish a shard convergence rate of the N-IHT estimator. (ii) Then, we establish the crucial restricted smoothness and restricted convexity properties of the squared error loss function under the bandit setting with high probability. These two results together yield the high probability convergence results of the N-IHT estimator. This estimation guarantee helps us to obtain a bound on the per-round regret. The rest of the analysis follows by summing up these per-round regrets over the time horizon.

%\textbf{Discussion of results:}
1. \textit{Dependence on $d, s, s^*,T$}: The term in $J(\epsilon, \delta)$ scaling as $\{(s + s^*)^3\log^2 d\}^{(1+\alpha)/2}$ dominates the non-private term $I_\alpha$ (for fixed $\epsilon, \delta$). The dependence on $T$ is trickier: for the non-private part, for $\alpha=0$, the regret scales as $\sqrt{T}$, for $\alpha=1$ as $\log T$ and the effect fades as $\alpha\to\infty$. For the private part $J_\alpha$, as $\alpha\to 0$, $\Psi_\alpha(T)$ can be upper bounded by $\log^3 T$, while the effect fades as $\alpha$ increases.      

2. \textit{Privacy trade-off for fixed $\alpha$}: For any fixed level of $\alpha$, the regret bound explicates the threshold of the privacy parameter $\epsilon$, under which the cost of privacy dominates the non-private term. For example, with $\alpha=0$ (no margin condition), $J_\alpha$ dominates $I_\alpha$ when $\epsilon/\sqrt{\log(1/\delta)} < \log^3 T\sqrt{\{(s+s^*)\log d\}/T}$. Similarly, for $\alpha=\infty$, the private part dominates when $\epsilon/\sqrt{\log(1/\delta)} < \sqrt{(s+s^*)\log d}$. 
     
3. \textit{Privacy vs. internal hardness}: An interesting feature arising in the reget analysis is the mutual struggle between the hardness coming from the bandit instance's arm-separation (through $\alpha$) and privacy constraint (through $\epsilon,\delta$). To understand this issue, let us denote $\bar{\epsilon}(\alpha)$ to be the threshold for $\epsilon$ under which the regret due to privacy dominates. We note that as $\alpha$ increases, $\bar{\epsilon}(\alpha)$ also increases, while keeping $\delta$ fixed. For example, $\bar{\epsilon}(\infty) = \sqrt{(s+s^*)\log d}\sqrt{\log(1/\delta)}$ and $\bar{\epsilon}(0) = \log^3 T\sqrt{\{(s+s^*)\log d\}\log(1/\delta)/T}$. Thus, when the bandit instance is easy, (high $\alpha$), the hardness due to the privacy is dominant for a larger range of $\epsilon$ (analogously high $\bar{\epsilon}(\alpha)$). Conversely, when the bandit instance is itself hard (low $\alpha$), the regret incurred due to this inherent difficulty quickly crosses the hardness due to privacy. As a result, even for smaller $\epsilon$, regret is dominated by the non-private part.

4. \textit{Achieving minimax optimal bound:} 
The regret bound in Theorem \ref{thm: regret} crucially depends on the quantity $(s+s^*)$. Therefore, the choice of $s$ is very important to avoid the curse of dimensionality. In a high-dimensional sparse setting, $s^*$ is typically very small, i.e., $s^* \ll d $. Therefore, setting $s $ in the order of $o(d)$ is also a valid choice, and an improved dependence on $d$ can be achieved. Moreover, under a constant order knowledge of $s^*$, the tuning parameter $s$ can be chosen as $s \asymp \kappa^2 s^*$ which leads to a near-optimal dependence in $s^*$. In addition, numerical experiments in Appendix~\ref{app: numerical s} show that the regret only scales polynomially in $s >s^*$ as shown in Theorem \ref{thm: regret}.
% \item \textit{Comparison with the lower bound}: We note that the terms involving $T, \epsilon, \delta$ in the private part of the upper bound matches the corresponding terms in the lower bound in Theorem \ref{thm:lb_edp} for all $\alpha\in (0,1)$. Thus, our algorithm enjoys an almost-minimax optimal regret bound for this range of $\alpha$, the suboptimality is in terms of $d$ - the private part of the lower bound has $(\log d)^{(1+\alpha)/2}$, while the upper bound is of the order $(\log d)^{1+\alpha}$ (in the term $J_{\alpha}(\epsilon,\delta)$ in Theorem \ref{thm: regret}), hence the lower bound is short by a factor of $(\log d)^{(1+\alpha)/2}$ in this case. ({ \textbf{Needs revision}})
% \end{enumerate}\vspace*{-.5em}

\vspace*{-.5em}\section{NUMERICAL EXPERIMENTS}\vspace*{-.5em}
We present an empirical study of the performance of FLIPHAT through several numerical experiments. All experiments were run locally on Macbook Pro with 16 GB RAM and 1.4 GHz Quad-Core Intel Core i5. 
Both of the experiments are setup in the problem-independent setting $\alpha=0$, and the plots show both the mean and $95\%$-CI for the mean (as colored bands) over 60 repetitions of each experiment. For space constraint, we present two of these experiments here, and postpone the additional details and studies to the Appendix \ref{sec: numerical details appendix}. 

In the first experiment, \textbf{we test the time evolution of regret of FLIPHAT}, and illustrate the regret against time $T$ in Figure \ref{fig: regret}(Left) in the case where $d=400, s^*=5, K=3$ up to $T=20000$ for different choices of privacy parameter $\epsilon\in\{0.5,1,2,5,10\}, \delta=0.01$. We also include \textit{random bandit} (taking random action at each time), which corresponds to $\epsilon=0$ (full privacy, no effective utility), and also the sparsity agnostic bandit \citep{oh2021sparsity}, which corresponds to $\epsilon\to\infty$, i.e. without any privacy guarantee, as the baselines. The contexts are drawn i.i.d. from $\cN(0,\Sigma)$, where $\Sigma_{ij}=0.1^{|i-j|}$ (autoregressive design), with observation noise being a centered Gaussian with $\sigma=0.1$. For the second experiment, \textbf{we illustrate the effect of context dimension $d$ on the regret suffered by FLIPHAT} at $T=10000$ for 4 different choices of $\epsilon$ (Figure \ref{fig: regret}-Right) in a setting similar to the first experiment, while $d$ takes 12 equi-spaced values from 400 to 4000.

\textbf{Results.} Figure~\ref{fig: regret} (Left) demonstrates the sublinear behavior of FLIPHAT's regret that approaches the sparsity agnostic bandit's regret for larger $\epsilon$. Figure~\ref{fig: regret} (Right) shows that $R(T)$ with $T=10000$ is nearly linear in $\log d$, where the slope $\beta$ (in the legend) is computed by fitting a linear model. This matches with the theoretical results in Theorem~\ref{thm: regret}, i.e., the cost of privacy in FLIPHAT scales as $O(\log d)$. 
%More details can be found in Appendix \ref{sec: numerical details appendix}.

% Now, we present numerical experiments to illustrate the sub-linear dependence of regret on the ambient dimension $d$ under different privacy budgets $\epsilon$. In these experiments, we vary $d$ from 400 to about 2800. We set $ s^*= 10, K = 3$ and $T = 30,000$. We generate the contexts across time and arms
% \begin{wrapfigure}{r}{0.45\textwidth}\vspace*{-1em}
\begin{figure}[t!]
\centering  \vspace*{-.5em}
  \includegraphics[width=\columnwidth]{aistats/plot_AR1e-1-s5-T40000-K3-gaussian-effect_d_new.pdf}\vspace*{-2em}
  \caption{(Left) Regret vs $T$ for different privacy level $\epsilon$, (Right) Regret at $T=10000$ vs $\log(d)$ for different $\epsilon$}\label{fig: regret}%\vspace*{-2em}
\end{figure}
% \end{wrapfigure}
% from the Autoregressive Gaussian design in an i.i.d. fashion and with parameter $\phi = 0.3$, i.e., $\Sigma_{ij} = 0.3^{\abs{i-j}}$ for $(i,j) \in [d]\times [d]$. Finally, the reward is generated according to the linear model (Equation~\eqref{eq: base model}) with Gaussian noise $N(0, 0.1)$. All experiments were run on an online cluster with 16 GB RAM and 8 CPU cores.
 
% This setup is the problem-independent setting, i.e. $\alpha = 0$, as no prior information about the arm-separation is available. 
% Figure~\ref{fig: regret} shows the final mean regret of FLIPHAT under $\delta =10^{-2}$ and $\epsilon \in \{0.8, 2, 5\}$ across 10 independent repetitions -- a 95\% confidence interval for the regret at each choice of $d$ is included in the figure as shaded bands around the mean regret lines. The dashed lines show that the regret depends almost logarithmically on the ambient dimension $d$. This matches with the theoretical results in Theorem~\ref{thm: regret}, i.e., the cost of privacy in FLIPHAT scales as $O(\log d)$. 
 
\vspace*{-.5em}\section{CONCLUSION}\vspace*{-.5em}
In this paper, we study the SLCBs under JDP constraints. 
We establish two minimax regret lower bounds under JDP settings, demonstrating phase transition between the hardness of the problem depending on the privacy level.
We propose FLIPHAT, which is the first algorithm to achieves sharp regret-privacy trade-off in SLCBs. FLIPHAT is based on the N-IHT algorithm, for which we propose a refined convergence analysis under a general setting than the existing literature.

% In particular, we establish novel minimax regret-bound results under JDP setting, demonstrating phase transition between the hardness of the problem depending on the privacy level. In addition, we propose a novel algorithm based on the doubling and forgetting trick that enjoys almost matching lower bounds in dimension, time horizon and privacy parameters under the JDP setting. 
% To the best of our knowledge, this is the first JDP algorithm that achieves sharp rates in the regret bound under SLCB setting. It is worthwhile to mention that our algorithm is based on the N-IHT algorithm, for which we propose a refined convergence analysis under a more setting compared to the existing literature. As a consequence, our algorithm can be deployed in time sensitive high-risk tasks such as mobile-health applications for which high-dimensional information becomes a bottleneck from both computation and privacy point of view.

% One natural extension of this work could be to explore the performance of FLIPHAT under the LDP setting, which is a stronger notion of privacy. Although, potentially the performance of FLIPHAT would be worse in the LDP setting compared to the JDP setting, it could be relevant in the field where the central server itself is not trusted. 
An interesting direction would be to study FLIPHAT under an adversarial sparse LCB setting. It would also be an interesting future study to explore the lower bound using the margin condition and obtain bounds dependent on the parameter $\alpha$ in the margin condition.

% There are a few natural open questions that arise from the present work. One future direction could be to establish minimax lower bound under $(\epsilon, \delta)$-DP constraints. Implementation of FLIPHAT and its comparison with private lasso-type algorithm is interesting research direction in this area.
